Functional Programming with Hypergraph Transformation

Complex data structures are difficult to manipulate declaratively while preserving their shape invariants. Functional languages offer pattern matching and strong static guarantees, but their type systems primarily describe tree-shaped data. Graph transformation languages support richer structures, yet their state-oriented models do not integrate naturally with value- and function-based programming. This dissertation introduces $\lambda_{GT}$, a functional language that integrates port-hypergraph transformation. It represents complex data as port hypergraphs, manipulates them by pattern matching, and uses types to specify global shape invariants. We formalise HyperLMNtal as a term-based graph transformation formalism, then define the syntax and call-by-value semantics of untyped $\lambda_{GT}$ and implement a prototype interpreter. We develop a core type system for $\lambda_{GT}$, prove its soundness, and relate it to graph-grammar-based typing. We extend the system with linear implication types to describe incomplete graphs arising during pattern matching. The extended system is sound with dynamic pattern-matching checks and is conservative over complete graph types. We also identify a statically safe fragment in which these checks can be eliminated. Finally, we mechanise the definitions and meta-theory in Isabelle/HOL.

==> images/fig-09-dbllist-2.tex <==
\begin{align}\label{eq:prod-rules-eg-vis-dbllist-2}
  \begin{array}{ccc}
    \dblltype{X}{Y}{Z}
     &
    \longrightarrow
     &
    \tikz[baseline=1.5ex, scale=1]{%
      \mknil{2}{(0,0)}
      %
      \node [link] (C1) at (-1, 0.8) {$Z$};
      \node [link] (LX) at (-1, 0.0) {$X$};
      \node [link] (C3) at (+1, 0.8) {$Y$};
      %
      \mkconslinkleft{1}{2}
      \draw (C2) to (LX);
      \mkconslinkright{2}{3}
    }
    \mid
    \tikz[baseline=1.5ex, scale=1]{%
      \mkcons{2}{W_1}{}{(0,0)}
      \mkdbll{3}{(1.5,0)}{W_2}
      %
      \node [link] (C1) at (-1.0, 0.8) {$Z$};
      \node [link] (LX) at (-1.0, 0.0) {$X$};
      \node [link] (C4) at (+2.5, 0.8) {$Y$};
      %
      \mkconslinkleft{1}{2}
      \draw (C2) to (LX);
      \mkconslink{2}{3}
      \mkconslinkright{3}{4}
    }
  \end{array}
\end{align}



==> images/fig-09.tex <==
\begin{align}\label{eq:prod-rules-eg-vis}
   & \Pdl \triangleq
  \notag             \\
   & \! \left\{
  \begin{array}{ccc}
    % Doubly-linked list
    \dblltype{X}{Y}{Z}
     &
    \longrightarrow
     &
    \tikz[baseline=-0.5ex, scale=1]{%
      \begin{scope}[shift={(0,0)}]
        \node [atom] (C1)  at (0, 0) {N};
        \coordinate (p1A) at ($(C1)+(0,0.4)$) {};
        \coordinate (p1R) at ($(p1A)+( 0.5,0.4)$);
        \coordinate (p1L) at ($(p1A)+(-0.5,0.4)$);
        \node [port] at (0.100, 0.400)   {2};
        \node [port] at (-0.400, -0.100) {1};
      \end{scope}
      %
      % Free links
      \node [link] (LZ) at (-1, 0.8) {$Z$};
      \node [link] (LX) at (-1, 0)   {$X$};
      \node [link] (LY) at (1, 0.8)  {$Y$};
      % Z
      \draw [in=180, out=0, looseness=1.50] (LZ) to (p1L);
      \draw [in=90, out=0, rounded corners] (p1L) to (p1A);
      \draw (p1A) to (C1);
      % X
      \draw (C1) to  (LX);
      % Y
      \draw [in=0, out=180, looseness=1.50] (LY) to (p1R);
      \draw [in=90, out=180, rounded corners]  (p1R) to (p1A);
    }
    \mid
    \tikz[baseline=-0.4ex, scale=1]{%
      \begin{scope}[shift={(0,0)}]
        \node [atom] (C1)  at (0, 0)    {C};
        \coordinate (p1A) at ($(C1)+(0,0.4)$) {};
        \coordinate (p1R) at ($(p1A)+( 0.5,0.4)$);
        \coordinate (p1L) at ($(p1A)+(-0.5,0.4)$);
        % \node [atom] (N1)  at ($(C1)+(0,-1)$) {1};
        \node [tvar] (N1)  at ($(C1)+(0,-1.1)$)  {$\mathit{n}$};
        \draw (C1) to (N1);
        \node [port] at (0.100, 0.450)   {4};
        \node [port] at (-0.450, -0.100) {2};
        \node [port] at (-0.100, -0.450) {1};
        \node [port] at (0.450, -0.100)  {3};
        \node [port] at (-0.100, -0.7)   {1};
        \node [link,text=gray] at (0.50, -0.6) {$(W_1)$};
      \end{scope}
      %
      \begin{scope}[shift={(1.5,0)}]
        % \node [atom] (C2)  at (0, 0)    {N};
        \node [tvar] (C2) at (0, 0) {$\mathit{dbll}$};
        \coordinate (p2A) at ($(C2)+(0,0.4)$) {};
        \coordinate (p2AL) at ($(C2)+(-0.2,0.3)$);
        \coordinate (p2AR) at ($(C2)+(+0.2,0.3)$);
        \coordinate (p2R) at ($(p2A)+( 0.6,0.4)$);
        \coordinate (p2L) at ($(p2A)+(-0.6,0.4)$);
        \node [port] at (-0.600, -0.100) {1};
        \node [port] at (+0.400, 0.450)  {2};
        \node [port] at (-0.400, 0.450)  {3};
        \node [link,text=gray] at (-0.400, 1.000)  {$(W_2)$};
      \end{scope}
      %
      % Free links
      \node [link] (LZ) at (-1, 0.8)  {$Z$};
      \node [link] (LX) at (-1, 0.0)  {$X$};
      \node [link] (LY) at (2.5, 0.8) {$Y$};
      %
      % Z
      \draw [in=180, out=0, looseness=1.50] (LZ) to (p1L);
      \draw [in=90, out=0, rounded corners] (p1L) to (p1A);
      \draw (p1A) to (C1);
      %
      % X
      \draw [port]  (C1) to  (LX);
      %
      % 1 -- 2
      \draw [in=180, out=0, looseness=1.50] (C1) to (p2L);
      \draw [in=90, out=0, rounded corners] (p2L) to (p2AL);
      \draw [line width=4pt,white,in=0, out=180, looseness=1.50] (C2) to (p1R);
      \draw [in=0, out=180, looseness=1.50] (C2) to (p1R);
      \draw [in=90, out=180, rounded corners]  (p1R) to (p1A);
      %
      % Y
      \draw [in=0, out=180, looseness=1.50] (LY) to (p2R);
      \draw [in=90, out=180, rounded corners]  (p2R) to (p2AR);
    }
    \\[6mm]
    % Natural number
    \tikz[baseline=1ex, scale=1]{%
      \node [tvar] (num1)  at (0, 0) {$\mathit{n}$};
      \draw (num1) --++ (0, 1);
      \node [link] at (0,     1.3) {$X$};
      \node [port] at (-0.25,  0.5) {1};
    }
     &
    \longrightarrow
    \tikz[baseline=1ex, scale=1]{%
      \node [atom] (num1) at (0, 0)    {1};
      \draw (num1) --++ (0, 1);
      \node [link] at (0,     1.3) {$X$};
      \node [port] at (-0.25,  0.5) {1};
    }
    \mid
    \tikz[baseline=1ex, scale=1]{%
      \node [atom] (num1) at (0, 0)    {2};
      \draw (num1) --++ (0, 1);
      \node [link] at (0,     1.3) {$X$};
      \node [port] at (-0.25,  0.5) {1};
    }
    \mid
    \dots
    \\[3mm]
    % Leaf-linked tree
    \lltrtype{X}{L}{R}
     &
    \longrightarrow
    \tikz[baseline=-2pt, scale=1]{%
      \node [atom]
      (cons1) at (0, 0) {L};
      \node [tvar] (num1)  at (0, -1.3) {$\mathit{n}$};
      \draw (cons1) -- (num1);
      %
      \coordinate (p1) at (+0.75, 0);
      \coordinate (p2) at (-0.75, 0);
      \coordinate (p3) at (0, 0.85) ;
      %
      \node [link] at (+0.85, 0) {$R$};
      \node [link] at (-0.85, 0) {$L$};
      \node [link] at (0, 0.95)  {$X$};
      %
      \draw(cons1) to (p1);
      \draw [looseness=1.50,in=30,out=90] (cons1) to (p2);
      \draw (cons1) -- (p3);
      %
      \node [port] at (0.200, 0.395)   {3};
      \node [port] at (0.395, 0.200)   {2};
      \node [port] at (-0.200, -0.395) {1};
      \node [port] at (-0.200, -0.7)   {1};
      %
      \node [link,text=gray] at (0.50, -0.7)   {$(W_1)$};
    }
    \mid
    \tikz[baseline=-2pt, scale=1]{%
      \node [atom,text=white,fill=black!60]
      (cons1) at (0, 0) {L};
      \node [tvar] (num1)  at (0, -1.3) {$\mathit{n}$};
      \draw (cons1) -- (num1);
      %
      \coordinate (p1) at (+0.75, 0);
      \coordinate (p2) at (-0.75, 0);
      \coordinate (p3) at (0, 0.85) ;
      %
      \node [link] at (+0.85, 0) {$R$};
      \node [link] at (-0.85, 0) {$L$};
      \node [link] at (0, 0.95)  {$X$};
      %
      \draw(cons1) to (p1);
      \draw [looseness=1.50,in=30,out=90] (cons1) to (p2);
      \draw (cons1) -- (p3);
      %
      \node [port] at (0.200, 0.395)   {3};
      \node [port] at (0.395, 0.200)   {2};
      \node [port] at (-0.200, -0.395) {1};
      \node [port] at (-0.200, -0.7)   {1};
      %
      \node [link,text=gray] at (0.50, -0.7)   {$(W_1)$};
    }
    \mid
    \tikz[baseline=5.4ex, scale=1]{%
      \begin{scope}[shift={(0,1.3)}]
        \node [atom] (cons1) at (0, 0) {N};
        %
        \node [port] at (0,     1.1) {$X$};
        \node [port] at (-0.2, 0.5) {$3$};
        \node [port] at (-0.2, -0.4) {1};
        \node [port] at ( 0.2, -0.4) {$2$};
      \end{scope}
      \draw (cons1) --++(0, 1);
      \begin{scope}[shift={(-0.75, 0)}]
        \node [lltr] (x1) at (0, 0) {$\mathit{lltr}$};
        %
        \node [link,text=gray] at (-0.1, 1.0) {$(W_1)$};
        \node [port] at (-0.25,  0.6) {$3$};
        \node [port] at (-0.5, 0.2) {1};
        \node [port] at ( 0.5, 0.2) {$2$};
      \end{scope}
      \begin{scope}[shift={(+0.75, 0)}]
        \node [lltr] (x2) at (0.0, 0) {$\mathit{lltr}$};
        %
        \node [link,text=gray] at (0.1, 1.0) {$(W_2)$};
        \node [port] at (-0.25,  0.6) {$3$};
        \node [port] at (-0.5, 0.2) {1};
        \node [port] at ( 0.5, 0.2) {$2$};
      \end{scope}
      \draw (cons1) -- ($(x1.north)-(0,0.1)$);
      \draw (cons1) -- ($(x2.north)-(0,0.1)$);
      \draw (x1) -- (x2);
      \draw (x1)--++(-1.0, -0.2);
      \draw (x2)--++( 1.0, -0.2);
      \node [link,text=gray] at (0, -0.4) {$(Y)$};
      \node [link] at (-1.9, -0.20) {$L$};
      \node [link] at (+1.9, -0.20) {$R$};
    }
  \end{array}\right.
\end{align}\relax



==> images/fig-depgraph-Core.tex <==
\begin{figure}
  \centering
  % \includegraphics[width=0.9\linewidth]{images/depgraph-Core}
  \includegraphics[width=0.4\linewidth]{images/depgraph-Core-dot}
  \caption{Dependency graph of the \lgt core formalisation.}
  \label{fig:depgraph-Core}
\end{figure}


==> images/fig-depgraph-LI.tex <==
\begin{figure}
  \centering
  % \includegraphics[width=0.9\linewidth]{images/depgraph-LI}
  \includegraphics[width=0.4\linewidth]{images/depgraph-LI-dot}
  \caption{Dependency graph of the \lgt formalisation with linear implications.}
  \label{fig:depgraph-LI}
\end{figure}


==> images/icgt2023/hypergraphs.tex <==
\begin{minipage}[b]{0.3\linewidth}
	\centering
	\begin{tikzpicture}[scale=1.1]
		\footnotesize
		\node [] (X) at (0, 0) {$X$};
		\node [atom] (n1) at (1, 0) {C};
		\node [above=0mm of n1] {$v_1$};
		\node [above left =-2mm and 0mm of n1] {$3$};
		\node [below right=-2mm and 0mm of n1] {$2$};
		\node [atom] (n2) at (2, 0) {N};
		\node [above=0mm of n2] {$v_2$};
		\node [above left =-2mm and 0mm of n2] {$1$};
		\draw (X)--(n1)--(n2);

		\node [below left =0mm and -2mm of n1] {$1$};
		\node [atom] (n3) at (1, -1) {$1$};
		\node [below=0mm of n3] {$v_3$};
		\node [above right=0mm and -2mm of n3] {$1$};
		\draw (n1)--(n3);
	\end{tikzpicture}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
	\centering
	\begin{tikzpicture}[scale=1.1]
		\footnotesize
		\node [] (X) at (0, 0) {$X$};
		\node [atom] (n1) at (1, 0) {C};
		\node [above=0mm of n1] {$v_1$};
		\node [above left =-2mm and 0mm of n1] {$3$};
		\node [below right=-2mm and 0mm of n1] {$2$};
		\node [atom] (n2) at (2, 0) {C};
		\node [above=0mm of n2] {$v_2$};
		\node [above left =-2mm and 0mm of n2] {$3$};
		\node [below right=-2mm and 0mm of n2] {$2$};
		\node [] (Y) at (3, 0) {$Y$};
		\draw (X)--(n1)--(n2)--(Y);

		\node [below left =0mm and -2mm of n1] {$1$};
		\node [atom] (n3) at (1, -1) {$1$};
		\node [below=0mm of n3] {$v_3$};
		\node [above right=0mm and -2mm of n3] {$1$};
		\draw (n1)--(n3);

		\node [below left =0mm and -2mm of n2] {$1$};
		\node [atom] (n4) at (2, -1) {$2$};
		\node [below=0mm of n4] {$v_4$};
		\node [above right=0mm and -2mm of n4] {$1$};
		\draw (n2)--(n4);
	\end{tikzpicture}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
	\centering
	\begin{tikzpicture}[scale=1.1]
		\footnotesize
		\node [] (X) at (0.5, 1) {$X$};
		\node [] (L) at (-0.2, 0) {$Y$};
		\coordinate[] (bowtie) at (0.5, 0);
		\node [atom] (n1) at (1, 0) {$\mathtt{Y}$};
		\node [above=0mm of n1] {$v_1$};
		\node [above left =-2mm and 0mm of n1] {$3$};
		\node [below right=-2mm and 0mm of n1] {$2$};
		\node [] (R) at (2, 0) {$Z$};
		\draw (X) to[out=-90,in=180] (bowtie);
		\draw (L)--(bowtie);
		\draw (bowtie)--(n1);
		\draw (n1)--(R);

		\node [below left =0mm and -2mm of n1] {$1$};
		\node [atom] (n3) at (1, -1) {$1$};
		\node [below=0mm of n3] {$v_2$};
		\node [above right=0mm and -2mm of n3] {$1$};
		\draw (n1)--(n3);
	\end{tikzpicture}
\end{minipage}


==> images/icgt2023/lltree.tex <==
\begin{tikzpicture}[scale=0.6]% [scale=0.5,framed]
  % \draw [draw=none, dotted] (-3.5, -8.5) grid (20, 15.5);

  \node [] (let) at (-2, 13.5) {$\mathbf{let}$};
  %
  \node [ctxn] (helper2) at (-0.5, 13.5) {$\mathit{map}$};
  \draw (helper2)--++(0, 1);
  %
  \node [ctxn] (f1) at (1.5, 13.5) {$f$};
  \draw (f1)--++(0, 1);
  %
  \node [triangle] (x1) at (3.5, 13.3) {$x$};
  \draw (x1)--++(-1, 0);
  \draw (x1)--++(1, 0);
  \draw (x1)--++(0, 1.2);
  %
  \node [] at (5.5, 13.5) {$=$};


  \node [] (letrec) at (-0.2, 11.5) {$\mathbf{let\ rec}$};
  %
  \node [ctxn] (helper2) at (2.0, 11.5) {$\mathit{helper}$};
  \draw (helper2)--++(0, 1);
  %
  \node [triangle, inner sep=0.8pt] (x1) at (4.5, 11.3) {$x'$};
  \draw (x1)--++(-1, 0);
  \draw (x1)--++(1, 0);
  \draw (x1)--++(0, 1.2);
  %
  \node [] at (6.5, 11.5) {$=$};

  \node [] (case) at (1, 9.5) {$\mathbf{case}$};

  \node [triangle, inner sep=0.8pt] (x1) at (3, 9.3) {$x'$};
  \draw (x1)--++(-1, 0);
  \draw (x1)--++(1, 0);
  \draw (x1)--++(0, 1.2);

  \node [] (of) at (4.9, 9.5) {$\mathbf{of}$};

  \begin{scope}[shift={(1, 0)}]
    \coordinate (t1) at (0.5 + 1, 5);
    \coordinate (t2) at (0.5 + 3, 8);
    \coordinate (t3) at (0.5 + 5, 5);
    \coordinate (t4) at (0.5 + 4.0, 5);
    \coordinate (t5) at (0.5 + 2.8, 7);
    \coordinate (t6) at (0.5 + 1.5, 5);
    \draw [fill=atomcolor, dashed, rounded corners]
    (t1)--(t2)--(t3)--(t4)--(t5)--(t6)--cycle;
    \node [] at (0.5 + 3.7, 6.3) {$y$};

    \node [atom] (l1) at (0.5 + 2.8, 5.5) {L};
    \node [atom] (m1) at (0.5 + 2.1, 4.5) {$\mathtt{M}$};
    \node [ctxn] (n1) at (0.5 + 3.3, 4.5) {$z$};
    \draw [rounded corners=3pt]
    (m1)--++(0, 1)--++(0.2, 0);
    % \draw (l1)--(m1);
    \draw (l1)--(n1);
    \draw (l1)--++(0.9, 0);
    \draw (l1)--++(-1, 0);
    \draw (l1)--++(0, 1.4);
    \draw (0.5 + 3, 7.9)--++(0, 0.5);
    \draw (0.5 + 1.3, 5.5)--++(-0.5, 0);
    \draw (0.5 + 4.7, 5.5)--++(0.5, 0);

    \node [] at (6.75, 6.3) {$\rightarrow$};

    \node at (8.9, 7.4) {$\mathbf{let}$};
    %
    \node [ctxn, inner sep=3pt] (n1) at (10, 7.4) {$z'$};
    \draw (n1)--++(0, 1);
    %
    \node at (11, 7.4) {$=$};
    %
    \node [ctxn] (n1) at (12, 7.4) {$f$};
    \draw (n1)--++(0, 1);
    %
    \node [ctxn] (n1) at (13.5, 7.4) {$z$};
    \draw (n1)--++(0, 1);
    %
    \node at (14.5, 7.4) {$\mathbf{in}$};


    \node [ctxn] (helper2) at (11, 4) {$\mathit{helper}$};
    \draw (helper2)--++(0, 1);

    \begin{scope}[shift={(2.5, 0)}]
      \coordinate (t1) at (2 + 9, 3);
      \coordinate (t2) at (2 + 11, 6);
      \coordinate (t3) at (2 + 13, 3);
      \coordinate (t4) at (2 + 12.0, 3);
      \coordinate (t5) at (2 + 10.8, 5);
      \coordinate (t6) at (2 + 9.5, 3);
      \draw [fill=atomcolor, dashed, rounded corners]
      (t1)--(t2)--(t3)--(t4)--(t5)--(t6)--cycle;
      \node [] at (2 + 11.7, 4.3) {$y$};

      \node [atom] (l1) at (2 + 10.8, 3.5) {L};
      \node [ctxn, inner sep=3pt] (n1) at (2 + 10.3, 2.5) {$z'$};
      \node [atom] (m1) at (2 + 11.5, 2.5) {$\mathtt{M}$};
      \draw [rounded corners=3pt]
      (m1)--++(0, 1)--++(0.2, 0);
      \draw (l1)--(n1);
      \draw (l1)--++(0.9, 0);
      \draw (l1)--++(-1, 0);
      \draw (l1)--++(0, 1.4);
      \draw (2 + 11, 5.9)--++(0, 0.5);
      \draw (2 + 9.3, 3.5)--++(-0.5, 0);
      \draw (2 + 12.7, 3.5)--++(0.5, 0);
    \end{scope}


    \node [] at (-0.5, 0.25) {$|$};

    \node [triangle] (x1) at (3.25, 0) {$y$};
    \draw (x1)--++(-1, 0);
    \draw (x1)--++(1.5, 0);
    \draw (x1)--++(0, 1.2);
    \node [atom] (m1) at (4.25, -1) {$\mathtt{M}$};
    \draw [rounded corners=3pt]
    (m1)--++(0, 1)--++(0.2, 0);

    \node [] at (6.75, 0.25) {$\rightarrow$};

    \node [triangle] (x1) at (9.5, 0) {$y$};
    \draw (x1)--++(-1, 0);
    \draw (x1)--++(1, 0);
    \draw (x1)--++(0, 1.2);
  \end{scope}

  \node [] (in) at (-0.7, -2) {$\mathbf{in}$};
  %
  \node [ctxn] (helper2) at (1, -3.5) {$\mathit{helper}$};
  \draw (helper2)--++(0, 1);
  %
  \node [triangle] (x1) at (4.5, -3.5) {$x$};
  \draw (x1)--++(-1.5, 0);
  \draw (x1)--++(1, 0);
  \draw (x1)--++(0, 1.2);
  %
  \node [atom] (m1) at (3.5, -4.5) {$\mathtt{M}$};
  \draw [rounded corners=3pt]
  (m1)--++(0, 1)--++(0.2, 0);


  \node [] (in) at (-2, -5.5) {$\mathbf{in}$};
  %
  \node [ctxn] (map2) at (-0.5, -7) {$\mathit{map}$};
  \draw (map2)--++(0, 1);
  %
  \node [atom] (f3) at (1.75, -7) {$+ 1$};
  \draw (f3)--++(0, 1);
  %
  \node [triangle] (x1) at (4, -7.2) {$t$};
  \draw (x1)--++(-1, 0);
  \draw (x1)--++(1, 0);
  \draw (x1)--++(0, 1.2);


  \draw [gray] (-2, -5)--++(0, 18);
  \draw [gray] (-2, -6)--++(0, -1.8)--++(0.3, 0);

  \draw [gray] (-0.7, -1.5)--++(0, 12.5);
  \draw [gray] (-0.7, -2.5)--++(0, -2.3)--++(0.3, 0);

  \draw [gray] (9.9, 6.9)--++(0, -5)--++(0.3, 0);
  % \draw [blue] (0.75, 9)--++(0, -7)--++(0.3, 0);
  % \draw [blue] (1.7, -3.4)--++(0, -1.5)--++(0.3, 0);

\end{tikzpicture}


==> images/icgt2023/lltrees.tex <==
\begin{tikzpicture}[scale=0.7]
  \begin{scope}[shift={(0, 0)}]

    \node [] (X) at (3, 4) {};
    \node [atom] (c1) at (3, 3)     {N};
    \node [atom] (c2) at (2, 2.5)   {N};
    \node [atom] (c3) at (4, 2.5)   {N};
    \node [atom] (c4) at (2.5, 1.5) {N};

    \draw (X)--(c1);
    \draw (c1)--(c2);
    \draw (c1)--(c3);
    \draw (c2)--(c4);

    \node [atom] (n1) at (1.1, 1.5) {L};
    \draw (c2)--(n1);
    \node [atom] (n2) at (2, 0.5)   {L};
    \draw (c4)--(n2);
    \node [atom] (n3) at (2.9, 0.5)   {L};
    \draw (c4)--(n3);
    \node [atom] (n4) at (3.8, 1.5) {L};
    \draw (c3)--(n4);
    \node [atom] (n5) at (4.7, 1.5) {L};
    \draw (c3)--(n5);

    \node [atom, below=1mm of n1] (ll1) {$1$};
    \draw (n1)--(ll1);
    \node [atom, below=1mm of n2] (ll2) {$2$};
    \draw (n2)--(ll2);
    \node [atom, below=1mm of n3] (ll3) {$3$};
    \draw (n3)--(ll3);
    \node [atom, below=1mm of n4] (ll4) {$4$};
    \draw (n4)--(ll4);
    \node [atom, below=1mm of n5] (ll5) {$5$};
    \draw (n5)--(ll5);

    \node [] (R) at (0.2, 1.5) {};
    \node [] (L) at (5.6, 1.5) {};
    \draw (R)--(n1) to[out=-20,in=160] (n2)--(n3) to[out=40,in=220] (n4)--(n5)--(L);

    % \node [] (label) at (3, -1.3) {\small (a)};
    \node [] (label) at (3, -1.7) {\small (a)};
  \end{scope}


  % \begin{scope}[shift={(10, 0)}]
  \begin{scope}[shift={(6, 0)}]

    \node [] (X) at (3, 4) {};
    \node [atom] (c1) at (3, 3)     {N};
    \node [atom] (c2) at (2, 2.5)   {N};
    \node [atom] (c3) at (4, 2.5)   {N};
    \node [atom] (c4) at (2.5, 1.5) {N};

    \draw (X)--(c1);
    \draw (c1)--(c2);
    \draw (c1)--(c3);
    \draw (c2)--(c4);

    \node [atom] (n1) at (1.1, 1.5) {L};
    \draw (c2)--(n1);
    \node [atom] (n2) at (2, 0.5)   {L};
    \draw (c4)--(n2);
    \node [atom] (n3) at (2.9, 0.5)   {L};
    \draw (c4)--(n3);
    \node [atom] (n4) at (3.8, 1.5) {L};
    \draw (c3)--(n4);
    \node [atom] (n5) at (4.7, 1.5) {L};
    \draw (c3)--(n5);

    \node [atom, below=1mm of n1] (ll1) {$2$};
    \draw (n1)--(ll1);
    \node [atom, below=1mm of n2] (ll2) {$3$};
    \draw (n2)--(ll2);
    \node [atom, below=1mm of n3] (ll3) {$4$};
    \draw (n3)--(ll3);
    \node [atom, below=1mm of n4] (ll4) {$5$};
    \draw (n4)--(ll4);
    \node [atom, below=1mm of n5] (ll5) {$6$};
    \draw (n5)--(ll5);

    \node [] (R) at (0.2, 1.5) {};
    \node [] (L) at (5.6, 1.5) {};
    \draw (R)--(n1) to[out=-20,in=160] (n2)--(n3) to[out=40,in=220] (n4)--(n5)--(L);

    % \node [] (label) at (3, -1.3) {\small (b)};
    \node [] (label) at (3, -1.7) {\small (b)};
  \end{scope}
\end{tikzpicture}

